Analysis of occupational and displacive disorder using the atomic pair distribution function: a systematic investigation

Many disordered crystalline materials show chemical short range order and relaxation of neighboring atoms. Local structural information can be obtained by analyzing the atomic pair distribution function (PDF). The viability of reverse Monte Carlo (RMC) simulations to extract quantitative information about chemical ordering as well as displacements is investigated. The method has been applied to simulated PDFs of disordered structures showing chemical disorder alone as well as in combination with displacements.

==> elements.tex <==
%Zeitschrift fuer Kristallographie, Oldenbourg Muenchen

\renewcommand{\Title}{Analysis of occupational and displacive disorder
                      using the atomic pair distribution function:
                      a systematic investigation}
\renewcommand{\AuthorsComplete}{Th. Proffen$^*$}

\renewcommand{\CorrespondenceAuthor}{(e-mail: proffen@pa.msu.edu)} 

\renewcommand{\InstitutionOne}
      {Department of Physics and Astronomy and Center for Fundamental
       Materials Research, \\ Michigan State University, East Lansing,
       MI 48824-1116, USA}   
 
\renewcommand{\InstitutionTwo}{}     %will appear under II
\renewcommand{\InstitutionThree}{}   %will appear under III 
\renewcommand{\InstitutionFour}{}    %will appear under IV 
\renewcommand{\InstitutionFive}{}    %will appear under V 
\renewcommand{\InstitutionSix}{}     %will appear under VI 

\renewcommand{\SayThanks}{This paper is dedicated to Prof. Dr. Heinz Schulz 
                          on the occasion of his 65th birthday.}

\renewcommand{\Abstract}
{ 
%
  Many disordered crystalline materials show chemical short range
  order and relaxation of neighboring atoms. Local structural
  information can be obtained by analyzing the atomic pair
  distribution function (PDF). The viability of reverse Monte Carlo
  (RMC) simulations to extract quantitative information about chemical
  ordering as well as displacements is investigated. The method has
  been applied to simulated PDFs of disordered structures showing
  chemical disorder alone as well as in combination with
  displacements.
%
} % includes the full abstract in English!


%%%%%%%%%%%%%%%%%%%%%%% for publisher only %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\Paperreceived}{} % date only; format: April 23, 1998
\renewcommand{\Paperaccepted}{} % date only; format: April 24, 1998
\setcounter{Papervolume}{215}   % publisher: volume number here
\setcounter{page}{1}            % publisher: pagenumber here

\renewcommand{\Authors}{Th. Proffen}

\renewcommand{\cleanTitle}{}   % only needed to eliminate additions from Title 
                               % like footnotes etc. for databank purposes
\renewcommand{\shortAuthors}{} % only needed for headings; else = Authors
\renewcommand{\shortTitle}{Analysis of occupational and displacive disorder
                           using the atomic pair distribution function}   
                               % only needed for headings; else = cleanTitle
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\endinput








